Metrizing Fairness

We study supervised learning problems that have significant effects on individuals from two demographic groups, and we seek predictors that are fair with respect to a group fairness criterion such as statistical parity (SP). A predictor is SP-fair if the distributions of predictions within the two groups are close in Kolmogorov distance, and fairness is achieved by penalizing the dissimilarity of these two distributions in the objective function of the learning problem. In this paper, we identify conditions under which hard SP constraints are guaranteed to improve predictive accuracy. We also showcase conceptual and computational benefits of measuring unfairness with integral probability metrics (IPMs) other than the Kolmogorov distance. Conceptually, we show that the generator of any IPM can be interpreted as a family of utility functions and that unfairness with respect to this IPM arises if individuals in the two demographic groups have diverging expected utilities. We also prove that the unfairness-regularized prediction loss admits unbiased gradient estimators, which are constructed from random mini-batches of training samples, if unfairness is measured by the squared $\mathcal L^2$-distance or by a squared maximum mean discrepancy. In this case, the fair learning problem is susceptible to efficient stochastic gradient descent (SGD) algorithms. Numerical experiments on synthetic and real data show that these SGD algorithms outperform state-of-the-art methods for fair learning in that they achieve superior accuracy-unfairness trade-offs -- sometimes orders of magnitude faster.

==> comments.tex <==
% for underbar
% \usepackage{amsmath}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{definition}[theorem]{Definition}
% % \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{remark}[theorem]{Remark}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{observation}[theorem]{Observation}
\newtheorem{assumption}[theorem]{Assumption}
% \newtheorem{example}[theorem]{Example}
% \newtheorem{axiom}[theorem]{Axiom}
%==================================


%======================================
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{equation*}\begin{aligned}}
\newcommand{\eea}{\end{aligned}\end{equation*}}
\newcommand{\ds}{\displaystyle}
\newcommand{\independent}{\protect\mathpalette{\protect\independenT}{\perp}}
\newcommand{\R}{\mathbb{R}}

\newcommand{\Max}{\max\limits_}
\newcommand{\Min}{\min\limits_}
\newcommand{\Sup}{\sup\limits_}
\newcommand{\Inf}{\inf\limits_}
\newcommand{\Tr}[1]{\Trace \big[ #1 \big]}

\newcommand{\wh}{\widehat}
\newcommand{\mc}{\mathcal}
\newcommand{\mbb}{\mathbb}
\newcommand{\inner}[2]{\big \langle #1, #2 \big \rangle }
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\cov}{\Sigma} % true covariance matrix
\newcommand{\covinv}{\Sigma^{-1}} % true precision matrix
\newcommand{\covsa}{\wh{\Sigma}} % covariance sample average

\newcommand{\PP}{\mbb P}
\newcommand{\Pnom}{\wh{\mbb P}}
\newcommand{\QQ}{\mbb Q}
\newcommand{\DD}{\mbb D}
\newcommand{\II}{\mc I}

\newcommand{\Struct}{\mc S} % structural set
\newcommand{\Ambi}{\mc P} % Ambiguity set
\newcommand{\Data}{\wh{\mc D}_n} % Data set
\newcommand{\DataKfold}{\wh{\mc D}}
\newcommand{\est}{X\opt} % DRO estimator for X
\newcommand{\estdual}{\dualvar\opt} % DRO estimator for lambda
\newcommand{\estx}{x\opt}
\newcommand{\LHSfunction}{\phi_\rho}
\newcommand{\dd}{\textrm{d}}
\newcommand{\lip}{\textrm{Lip}}


%\newcommand{\est}{X\opt}
%\newcommand{\estL}{\lambda\opt}
%\newcommand{\estx}{x\opt}

\DeclareMathOperator{\Trace}{Tr}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Diag}{Diag}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\st}{s.t.}
\DeclareMathOperator{\nullspace}{null}
\DeclareMathOperator{\vect}{vec}
\DeclareMathOperator{\KL}{KL}
\DeclareMathOperator{\FR}{FR}
\DeclareMathOperator{\Argmin}{Argmin}
\DeclareMathOperator{\Minval}{Min}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\Hess}{Hess}
\newcommand{\eye}{\mathbb{I}}

\newcommand{\lip}{\textrm{Lip}}

\newcommand{\defeq}{%
  \mathrel{\vbox{\offinterlineskip\ialign{%
    \hfil##\hfil\cr
    $\scriptscriptstyle\triangle$\cr
    %\noalign{\kern0ex}
    $=$\cr
}}}}

% Peyman's comments
\newcommand{\PSD}{\mathbb{S}_{+}} % the set of positive semi-definite matrices of dimension p
\newcommand{\PD}{\mathbb{S}_{++}} % the set of positive semi-definite matrices of dimension p
\newcommand{\Let}{\triangleq}
\newcommand{\opt}{^\star}
\newcommand{\eps}{\varepsilon}
\newcommand{\ra}{\rightarrow}
\newcommand{\M}{\mc M}
\newcommand{\BB}{\mbb B}
\newcommand{\B}{\mc B}
\newcommand{\X}{X}
\newcommand{\Y}{Y}
\newcommand{\Wass}{\mathds{W}}
\newcommand{\V}{\mathds{W}_S}
\newcommand{\Q}{\mbb{Q}}
\newcommand{\EE}{\mathds{E}}
\newcommand{\tr}{\intercal}
\newcommand{\Xset}{\mc X}

\newcommand{\half}{\frac{1}{2}}
\newcommand{\dualvar}{\kappa}

\newcommand{\auxfunc}{\omega}
\newcommand{\covsaeig}{\lambda}
\newcommand{\covsaeigvect}{v}
\newcommand{\ie}{{\em i.e.}}
\newcommand{\da}{\downarrow}
\newcommand{\J}{\mc J}
\newcommand{\Dataset}{\wh{\mc D}}

\newcommand{\p}{\mathbb P}
\newcommand{\psa}{\wh \p}
\newcommand{\N}{\mathcal N}
\newcommand{\f}{f}
\newcommand{\g}{g}
\newcommand{\radius}{\rho}
\newcommand{\Sym}{\mbb S}
\newcommand{\m}{\mu}
\newcommand{\msa}{\wh \m}



==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> style.tex <==
% ================== Margins & Layout =================================
\addtolength{\voffset}{0cm} 
\addtolength{\textheight}{1cm} 
\addtolength{\hoffset}{-2cm}
\addtolength{\textwidth}{4cm}

\setlength{\parskip}{1mm}
\linespread{1.12}


%================================ Packages =====================================
%\usepackage[round]{natbib}
\usepackage{mathtools}
\usepackage{xr-hyper}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\usepackage{amssymb, bbm}
\usepackage{dsfont, mathrsfs, color, enumitem, url}
\usepackage{transparent, wrapfig}
\usepackage{float}
\usepackage{placeins}
\usepackage{subcaption}
%\usepackage[ruled,vlined]{algorithm2e}
% \usepackage{titlesec}
\usepackage{tcolorbox}
\usepackage{multicol}
%\usepackage{algorithm2e}
\usepackage{algorithm, algorithmic}
\renewcommand{\algorithmicrequire}{\textbf{Input:}} 
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\renewcommand{\algorithmiccomment}[1]{\hfill\ttfamily{// #1}}
\usepackage{bbm}


% \titlelabel{\thetitle.\;}
%===============================================================================

%============================== Abbreviation ===================================
\DeclareMathOperator{\Trace}{Tr}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\newcommand{\note}[1]{{\color{red}{Note: #1}}}


\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Cov}{\mathrm{Cov}}

\newcommand{\Pnom}{\hat \PP} 
\newcommand{\supp}{\textrm{supp}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\Max}{\max\limits_}
\newcommand{\Min}{\min\limits_}
\newcommand{\Sup}{\sup\limits_}
\newcommand{\Inf}{\inf\limits_}
\newcommand{\mbb}{\mathbb}
\newcommand{\Wass}{\mathds W}
\newcommand{\RR}{\mathds R}
\newcommand{\opt}{^\star}
\newcommand{\inner}[2]{\big \langle #1, #2 \big \rangle }
\newcommand{\ds}{\displaystyle}

\newcommand{\defeq}{\coloneqq}

\newcommand{\ie}{\textit{i.e., }}
\newcommand{\R}{\mathbb{R}}
\newcommand{\wh}{\widehat}
\newcommand{\dist}{\textrm{\textbf{dist}}}
\newcommand{\mc}{\mathcal}
\newcommand{\dd}{\mathrm{d}}

\newcommand{\EE}{\mathds{E}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\lip}{\textrm{Lip}}

\newcommand{\PP}{\mathbb{P}}
\newcommand{\x}{\mathcal{X}}
\newcommand{\y}{\mathcal{Y}}
\newcommand{\asinh}{\textrm{arcsinh}}
\newcommand{\samplerate}{\mathcal{O}}
\newcommand{\cdf}{F}
\newcommand{\bs}{\boldsymbol}
\newcommand{\ctransj}{\dvy_j-c(x,y_j)}
\newcommand{\ctransjneg}{-\dvy_j+c(x,y_j)}
\newcommand{\euler}{\gamma}
\newcommand{\DS}{\displaystyle}
\newcommand{\st}{\mathrm{s.t.}}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\eps}{\varepsilon}
\newcommand{\cov}{\Sigma} % true covariance matrix
\newcommand{\covsa}{\wh{\cov}}
\newcommand{\m}{\mu}
\newcommand{\msa}{\wh \m}
\newcommand{\dualvar}{\gamma}
\newcommand{\Sym}{\mathbb{S}}
\newcommand{\PSD}{\mathbb{S}_{+}} % the set of positive semi-definite matrices of dimension p
\newcommand{\PD}{\mathbb{S}_{++}} % the set of positive semi-definite matrices of dimension p
\newcommand{\Let}{\triangleq}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\Tr}[1]{\Trace \big[ #1 \big]}
\newcommand{\odd}{\mathrm{odd}}
\newcommand{\opp}{\mathrm{opp}}
\newcommand{\eye}{\mathbb{I}}
\newcommand{\acc}{\textgoth{A}}

%===============================================================================

%================================ Theorem ======================================
\theoremstyle{definition}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
%===============================================================================


%============================== Figures Path ===================================
\graphicspath{{figures/}}
%===============================================================================

%============================== Modify style ===================================
%\usepackage[utf8]{inputenc}    % allow utf-8 input
%\usepackage[T1]{fontenc}       % use 8-bit T1 fonts
\usepackage{tabularx}
%\usepackage{lmodern}           % allow pdf compability
\usepackage{xcolor}
% \hypersetup{
% 	colorlinks,
% 	linkcolor={blue!55!black},
% 	citecolor={red!55!black},
% 	urlcolor={blue!80!black}
% }
% \usepackage[a4paper, total={7in, 10in}]{geometry}
%===============================================================================

\usepackage{multicol}
\usepackage{algorithm}
\usepackage{multirow}
\usepackage{amsfonts}

% ================== Margins & Layout =================================
%\usepackage[a4paper, total={7.5in, 10.5in}]{geometry}
%\usepackage{setspace}
%\doublespacing

% \addtolength{\voffset}{0cm} 
% \addtolength{\textheight}{1cm} 
% \addtolength{\hoffset}{-2cm}
% \addtolength{\textwidth}{4cm}

% \setlength{\parskip}{1mm}
% \linespread{1.12}


